Fast and accurate method for computing non-smooth solutions to constrained control problems

Introducing flexibility in the time-discretisation mesh can improve convergence and computational time when solving differential equations numerically, particularly when the solutions are discontinuous, as commonly found in control problems with constraints. State-of-the-art methods use fixed mesh schemes, which cannot achieve superlinear convergence in the presence of non-smooth solutions. In this paper, we propose using a flexible mesh in an integrated residual method. The locations of the mesh nodes are introduced as decision variables, and constraints are added to set upper and lower bounds on the size of the mesh intervals. We compare our approach to a uniform fixed mesh on a real-world satellite reorientation example. This example demonstrates that the flexible mesh enables the solver to automatically locate the discontinuities in the solution, has superlinear convergence and faster solve times, while achieving the same accuracy as a fixed mesh.

==> Results/blockMove.tex <==
%Responsible: Eduardo
One is concerned with moving a block across a frictionless surface of unit length in minimum time, similar to minimum force or minimum work variants\cite{kelly_introduction_2017}. The block is controlled by an input force $u(\cdot) \in [-4, 4]$ which affects its velocity $v(\cdot)$ and, in turn, its position $x(\cdot)$ along the surface. Despite the continuous (linear) dynamics,
\begin{equation}
\begin{aligned}
    \dot{x}(t) &= v(t),\\
    \dot{v}(t) &= u(t),
\end{aligned}
\end{equation}
for the boundary conditions
\begin{equation}
\begin{aligned}
    x(0) & = 0, \quad x(t_f) = 1,\\
    v(0) & = 0, \quad v(t_f) = 0,\\
\end{aligned}
\end{equation}
the minimum-time solution $t_f = 1$ has a discontinuity in $u(0.5)$. The problem is restricted to a DAE with $x(\cdot)$ and $v(\cdot)$ as differential variables, and $u(\cdot)$ as an algebraic variable, defined over $t \in [0, 1]$. Fixed and flexible mesh schemes were used by our integrated residuals solver.
\begin{comment}
Given the nature of the problem, any uniform mesh with even-number intervals would \emph{accidentally} capture the discontinuity. This was circumvented by using odd number intervals ($N \in [3, 101]$).\\
\end{comment}
%
Three intervals were sufficient for the quasi-flexible scheme to capture the discontinuity at $t=0.5$, its solving time was analysed for a range of integrated residual tolerances. A performance comparison is shown in Figure~\ref{fig:blockMovePerformance} where mean solve times for both mesh types are plotted against the integrated residuals.
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Results/blockMovePerformance.pdf}
    \caption{Performance comparison of mesh schemes for block-move solution.}
    \label{fig:blockMovePerformance}
\end{figure}
For an integrated residual tolerance of $10^{-7}$ the flexible scheme is four times faster, and for a solve time of $1\,s$, it achieves two orders of magnitude higher accuracy.

==> Results/dde.tex <==
Consider the following non-autonomous ODE
\begin{equation}
    \dot{x}(t) =
    \begin{cases}
      1 \quad &\text{if $0 \leq t \leq 1$}\\
      e^{t-1} - 1 \quad &\text{if $1 < t \leq 2$}
    \end{cases},
    \quad \forall t \in [0, 2],
\label{eq:dde}
\end{equation}
where $x : \mathbb{R} \rightarrow \mathbb{R}$ is a (piecewise-differential) dynamic variable. By inspection, one expects the discontinuity in $\dot{x}(1)$ to result in a kink in $x(1)$.

Fixed and flexible mesh schemes were used by our integrated residuals solver. Results for different number of mesh intervals ($N$) are shown on Figure~\ref{fig:ddeConvergence}. Here the integrated residuals are plotted against $1/N$ so as to analyse the convergence of each scheme. Linear fits report slopes of 0.9258 and 3.6785, respectively for fixed and flexible meshes.

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{Results/daeConvergence.pdf}
    \caption{Convergence of fixed and flexible mesh solutions to (\ref{eq:dde})}
    \label{fig:ddeConvergence}
\end{figure}

==> legacy.tex <==
%This paper will explore integrated residual method as an alternative to collocation. Using our approach, one is effectively solving an unconstrained problem that guarantees dynamic constraints satisfaction and can heavily benefit from warm starting. Additionally, the concept of quasi-flexible mesh was implemented and it has been shown that the accuracy of the solution can be improved by including the mesh nodes as decision variables for the optimization problem. Compared to a fixed, pre-defined mesh, our strategy can capture discontinuities in the solution since nodes naturally migrate to regions of high gradients, as it will be proved in this paper. Lastly, we present some numerical examples to demonstrate the strength of our algorithm which can potentially be extended to solving challenging control problems with dynamic constraints formulated as a set of differential algebraic equations.  

%
%
%


- Existing numerical methods used in solving dynamic optimization problems can be classified in two broad categories: one can either first-discretize-then-optimize (as it is the case for direct methods), or first-optimize-then-discretize (as it is done in indirect methods). One popular approach is represented by direct collocation which uses polynomial basis functions to approximate the state on each mesh interval. 

To compute the approximating polynomials, collocation methods try to make the residual vanish at a finite set of values (also called collocation points or nodes). In contrast, our approach relies on numerically integrating the least-squares residual over the whole domain and then minimizing the integrated residual to construct the approximating basis functions. 

Compared to classical time-marching schemes (shooting methods) or fixed points residual minimization (collocation), integrated residual methods have the benefit of producing a solution of uniform quality over the whole time domain. 

\begin{comment}
\section{Legacy RESULTS}
\begin{itemize}
    \item A discontinuous DAE with a continuous solution;
    \item An optimal control problem whose solution is discontinuous at non-trivial locations.
\end{itemize}
    
\subsection{Linear ODE example}
Using 3rd degree Lagrange polynomials, with appropriate quadrature order,
\begin{equation}
    \frac{dx}{dt} = -x, x_0 = 1.0, t[0.0, 3.0]
    \label{eq:ode}
\end{equation}
was solved on a fixed, and 
The residual error is shown on Figure \ref{fig:odeResidual}.
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{odeResidual.png}
    \caption{Local residual error}
    \label{fig:odeResidual}
\end{figure}

In order to test for convergence, (\ref{eq:ode}) was solved for stage numbers [3, 10, 30, 100]
\begin{equation}
    r \leq K\bigg(\frac{\Delta t}{N}\bigg)^p
\end{equation}
\begin{equation}
    \log(r) \leq \log(K) + p \log\bigg(\frac{\Delta t}{N}\bigg)
\end{equation}
The convergence Figure \ref{fig:odeLogLog}
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{odeLogLog.png}
    \caption{Convergence}
    \label{fig:odeLogLog}
\end{figure}

\subsection{Optimal control example}
The minimum-work block-move example [cite Kelly] is used. Despite its continuous, linear dynamics, the solution.
\begin{equation}
    \begin{aligned}
        \min_{x_1(\cdot),x_2(\cdot),u(\cdot)} \quad & \int_0^1 |u(t) x_2(t)| \diff{t} \\
        \textrm{s.t.} \quad & \dot{x}_1 = x_2,\\
                            & \dot{x}_2 = u,\\
                            & -u_{max} \leq u \leq u_{max},\\
                            & x_1(0) = x_2(0) = \dot{x}_2 = 0,\\
                            & x_1(1) = 1.
    \end{aligned}
\end{equation}
The analytical solution is given by
\begin{equation}
    \begin{aligned}
        & u^{*}(t)=\left\{\begin{array}{ll}
            u_{\max ,} & t<t^{*} \\
0 & \text { otherwise } \\
-u_{\max }, & \left(1-t^{*}\right)<t
\end{array}\right.\\
&\text { where }\\
&t^{*}=\frac{1}{2}\left(1-\sqrt{1-\frac{4}{u_{\max }}}\right)
\end{aligned}
\end{equation}

Setting $u_{max} = 8$
\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\columnwidth]{example-image-c}
    \caption{solution}
    \label{fig:ocpSolution}
\end{figure}

The convergence Figure \ref{fig:ocpLogLog}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\columnwidth]{example-image-b}
    \caption{Convergence}
    \label{fig:ocpLogLog}
\end{figure}
\end{comment}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section*{APPENDIX}

%Appendixes should appear before the acknowledgment.

%\section*{ACKNOWLEDGMENT}

%The preferred spelling of the word ÒacknowledgmentÓ in America is without an ÒeÓ after the ÒgÓ. Avoid the stilted expression, ÒOne of us (R. B. G.) thanks . . .Ó  Instead, try ÒR. B. G. thanksÓ. Put sponsor acknowledgments in the unnumbered footnote on the first page.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.

\begin{comment}
\hl{The following things might be redundant, everybody knows about Lagrange basis I assume. The rest still needs to be formalized.}

Given $approxOrder$ ($aO$) internal nodes used for approximating the state on interval $t\in[t_i,t_{i+1}]$ with a Lagrange polynomial of degree $approxOrder-1$ ($aO-1$) the basis functions are: 
\begin{equation}
    \tilde{x}(t,[...s_i...],[...t^*_i...])=\sum_{i=1}^{aO}{\prod_{\substack{j=1 \\ j\neq i}}^{aO}{\frac{t-t^*_j}{t^*_i-t^*_j}\cdot s_i}}
\end{equation}
where $t$ represents the time evaluation point, $t^*_i$ represents the $i^{th}$ internal mesh node and $s_i$ is the $i^{th}$ decision variable.

Similarly we can define state derivative as
\begin{equation}
    \dot{\tilde{x}}(t,[...s_i...],[...t^*_i...])=\sum_{i=1}^{aO}{\sum_{\substack{k=1\\ k\neq i}}^{aO}{\frac{1}{t^*_i-t^*_j}\prod_{\substack{j=1\\ j\neq i\\ j\neq k}}^{aO}{\frac{t-t^*_j}{t^*_i-t^*_j}\cdot s_i}}}
\end{equation}

The partial derivatives with respect to our decision variables $s_i$ are 
\begin{equation}
    \frac{\partial\tilde{x}}{\partial s_i}(t,[...s_i...],[...t^*_i...])=\prod_{\substack{j=1 \\ j\neq i}}^{aO}{\frac{t-t^*_j}{t^*_i-t^*_j}}
\end{equation}
\begin{equation}
    \frac{\partial\dot{\tilde{x}}}{\partial s_i}(t,[...s_i...],[...t^*_i...])=\sum_{\substack{k=1\\ k\neq i}}^{aO}{\frac{1}{t^*_i-t^*_j}\prod_{\substack{j=1\\ j\neq i\\ j\neq k}}^{aO}{\frac{t-t^*_j}{t^*_i-t^*_j}}}
\end{equation}

As in any semi-infinite programming problem, we use basis functions to reduce the problem and only compute the solution at a finite number of discretization points (nodes). For point $p \in \{1,\dots,aO\}$ of state dimension $d\in \{1,\dots,D\}$ and interval $i \in \{1,\dots,N\}$ we have a decision variable indexed as: $s_{(i-1)*dim*aO+(d-1)*aO+p}$.
\end{comment}

\begin{comment}

Under the same assumption of subnodes existing on the boundaries, the initial condition (state) is introduced by 
\begin{equation}
    s_{(d-1)*aO+1}=x0_d \, \forall d \in \{1, \dots, dim\}
\end{equation}

As a result, we will have $m=N*dim$ constraints enforced as $g(s)=0$ where $g$ is a column vector defined as follows:
\begin{align*}
    &g_{(i-1)*dim+d}(s)=\\
    &s_{(i-1)*dim*aO+(d-1)*aO+aO} - s_{i*dim*aO+(d-1)*aO+1}\\
    &\forall i \in {1,\dots,N-1}\, \forall d \in {1,\dots,dim} 
\end{align*}
\begin{align*}
    &g_{(N-1)*dim+d}(s)=s_{(d-1)*aO+1} - x0_d \, \forall d \in {1,\dots,dim} 
\end{align*}

By computing the Jacobian of the constraint function \textbf{g} with respect to decision variable vector \textbf{s} we get:
\begin{align*}
    &(\nabla g)_{(i-1)*dim+d, \, (i-1)*dim*aO+(d-1)*aO+aO}=1\\
    &(\nabla g)_{(i-1)*dim+d, \, i*dim*aO+(d-1)*aO+1}=-1\\
    &\forall i \in {1,\dots,N-1}\, \forall d \in {1,\dots,dim}
\end{align*}
\begin{align*}
    &(\nabla g)_{(N-1)*dim+d,(d-1)*aO+1}=1\, \forall d \in {1,\dots,dim} 
\end{align*}

Hessian of the each constraint function $g_i$ with respect to decision variable vector \textbf{s} is equal to the zero matrix for all $i \in \{1,\dots,m\}$:
\begin{equation}
     \nabla^2 g_i = 0_{N*dim*aO\times N*dim*aO} \, \forall i \in \{1,\dots,m\}
\end{equation}
As a direct consequence, the hessian of the Lagrangian will be equal to the Hessian of the objective function. 

To obtain the gradient of the objective function $\nabla obj(s)$ we need to perform the following computation:
\begin{align}
    \nabla obj(s)=\sum_{i=0}^{N-1}{\sum_{d=1}^{D}{\sum_{q=1}^{qO}{2\cdot w_{q,i}\cdot F_d(\dot{x},x)\cdot \nabla F_d(\dot{x},x)}}}
\end{align}

\begin{align}
    \nabla  F_d(\dot{x}(t_{q,i},s),x(t_{q,i},s))=\frac{dF_d}{ds}=\frac{\partial F_d}{\partial \dot{x}}\frac{\partial \dot{x}}{\partial s}+\frac{\partial F_d}{\partial {x}}\frac{\partial {x}}{\partial s}
\end{align}

Similarly, to obtain the hessian of the objective function we get:
\begin{align}
    \nabla^2 obj(s)=\sum_{i=0}^{N-1}{\sum_{d=1}^{D}{\sum_{q=1}^{qO}{2\cdot w_{q,i}( (\nabla F_d)^2 + (F_d\cdot \nabla^2 F_d))}}}
\end{align}

\begin{align}
    \nabla^2 F_d(\dot{x}(t_{q,i},s),x(t_{q,i},s))=\frac{\partial^2 F_d}{\partial \dot{x}^2}(\frac{\partial \dot{x}}{\partial s})^2+\frac{\partial^2 F_d}{\partial {x}^2}(\frac{\partial {x}}{\partial s})^2+\\
    +2\frac{\partial^2 F_d}{\partial \dot{x} \partial x}\frac{\partial \dot{x}}{\partial s}\frac{\partial {x}}{\partial s}
\end{align}

\end{comment}


\begin{comment}
\begin{algorithm}
\SetAlgoLined
\KwResult{$t^*(t_i,t_{i+1}), t^* \in \mathbb{R}^{approxOrder}, t_i,t_{i+1}\in\mathbb{R}$}
 $\Delta=\frac{t_{i+1}-t_i}{approxOrder-1}$\;%Define step for equidistant mesh
 
 \For{While condition}{
  instructions\;
  \eIf{condition}{
   instructions1\;
   instructions2\;
   }{
   instructions3\;
  }
 }
 \caption{How to write algorithms}
\end{algorithm}
\end{comment}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{example-image-c}
%     \caption{Solution interpolation and mesh definition}
%     \label{fig:Meshdef}
% \end{figure}

%\section{MAIN RESULTS}
%\subsection{Problem structure}% for fixed mesh IRM}
%\begin{theorem}
%Problem BLA has the following structure.
%\end{theorem}

%\subsection{Quasi-flexible mesh}
%\begin{theorem}
%Minimizing (cost) with respect to x,u,t <= Minimizing (same cost) with respect to x,u. Results better accuracy for fixed mesh.
%\end{theorem}

%\begin{theorem}
%When using a flexible mesh, nodes $t_i$ will be located at the points of highest gradient from each allowed flexibility interval.
%\end{theorem}


%
%\subsection{Dynamics constraints in optimization-based control}
%Define J, F, x etc



%\subsection{Integrated Residual Methods}


    %\min_{x,u,t_i} \quad J(x,u,t) +
    %\sum_{i=0}^{N-1}{\sum_{q=1}^{qO}{w_{q,i}\cdot\sum_{d=1}^{D}{ F_d^2(\dot{x}(),x(),u(),t_{q,i})}}}\\
    %\sum_{d=1}^{D}{F_d(\frac{\diff{x}}{\diff{t}},x,u,t)^2}\\
    
    
    
    
%\begin{figure}[!tbp]
%\psfrag{uti}[][]{$\tilde{u}(t)$}
%\psfrag{uu}[][]{$u_U$}
%\psfrag{ul}[][]{$u_L$}
%\psfrag{t0}[][]{$t_{0}$}
%\psfrag{t1}[][]{$t_1$}
%\psfrag{t2}[][]{$t_2$}
%\psfrag{t3}[][]{$t_3$}
%\psfrag{t}[][]{$t$}
%\psfrag{t1ms}[][]{{$t_1-\sigma$}}
%\psfrag{t1ps}[][]{{$t_1+\sigma$}}
%\psfrag{t2ms}[][]{{$t_2-\sigma$}}
%\psfrag{t2ps}[][]{{$t_2+\sigma$}}
%\psfrag{sp}[][]{$\shortparallel$}
%\psfrag{t40}[][]{{$t_1^{\#}$}}
%\psfrag{t41}[][]{{$t_2^{\#}$}}
%\psfrag{tnn1}[][]{$t_{N}$}
%\centering
%\includegraphics[width=0.48\textwidth]{Fig31.pdf}
%\caption[Notation]{Fig 3. Solid - flexible mesh, dashed - fixed mesh, dotted - analytic}
%\label{fig:NotationFig3}
%\end{figure}

% \begin{figure}[!tbp]
% \psfrag{uti}[][]{$\tilde{u}(t)$}
% \psfrag{uu}[][]{$u_U$}
% \psfrag{ul}[][]{$u_L$}
% \psfrag{t0}[][]{$t_{0}$}
% \psfrag{t1}[][]{$t_1$}
% \psfrag{t2}[][]{$t_2$}
% \psfrag{t3}[][]{$t_3$}
% \psfrag{t}[][]{$t$}
% \psfrag{t1ms}[][]{{$t_1-\sigma$}}
% \psfrag{t1ps}[][]{{$t_1+\sigma$}}
% \psfrag{t2ms}[][]{{$t_2-\sigma$}}
% \psfrag{t2ps}[][]{{$t_2+\sigma$}}
% \psfrag{sp}[][]{$\shortparallel$}
% \psfrag{t40}[][]{{$t_1^{\#}$}}
% \psfrag{t41}[][]{{$t_2^{\#}$}}
% \psfrag{tnn1}[][]{$t_{N}$}
% \centering
% \includegraphics[width=0.48\textwidth]{Fig22}
% \caption[Notation]{Fig 2}
% \label{fig:NotationFig2}
% \end{figure}

%%%
\begin{comment}
To construct a solution to problem \eqref{eq:unconstrained_pb} we first need to discretize the space $\mathcal{T}$ into a  the 
\end{comment}

%%%%%%%%%%%%%%%
% 
%%%%%%%%%%%%%%%
\begin{comment}
Let us consider a control problem with states $x(\cdot)$, inputs $u(\cdot)$, dynamics $\dot{x}(\cdot)$, continuous time variable $t$ and cost functional $J(\cdot)$ having dynamics constraints in the form of a set of differential algebraic equations (DAEs) as in \eqref{eq:ctrl_problem}.

\begin{equation}
    \begin{aligned}
        \min_{x,u} \quad & J(x,u,t)\\
        \textrm{s.t.} \quad & F(\dot{x}, x, u, t) = 0 \ \  \forall t\in[t_0,t_f]\\
        %& 0=F(\frac{\diff{x}}{\diff{t}},x,u,t)\\
        %& 0 \geq g(\frac{\diff{x}}{\diff{t}},x,u,t)
    \end{aligned}
    \label{eq:ctrl_problem}
\end{equation}


and solve a least squares problem. the solution of equation. 
\end{comment}

%, or even aid individuals in taking management decisions


\begin{comment}
Intro: 
%Existing methods used in solving....<here goes the bit about collocation and why it fails, multiple shooting and why it fails, existing meshing and why it fails, time-marching bits as well>.

% combining benefit of quasi-flexible mesh with the integrated residual approach, hence having ability to ensure accuracy for trajectories in-between mesh nodes as they move around. 

%Differential equations have a central role in many applications ranging from engineering electrical circuits and fluid dynamics modelling to structural analysis and even medical imaging. 
%Once stated, these equations are used as a building block in control problems to compute an optimal set of inputs to a dynamical system.


% Since early ages, researchers wanted to formally describe the time-evolution of the physical world. Over the years, many systems and processes were treated as a set of differential equations modelling the input-output behaviour. Due to high complexity, most real-life equations cannot be solved analytically which justifies the need for fast and accurate numerical solvers. Developing numerical methods that are able to solve complex differential equations has been an active field of research within mathematical and scientific communities for many decades. In this paper, we approach the topic from a control engineering perspective and we propose a new method to solve differential equations in the context of control-related applications and problems.
% \hl{Our strategy is using least squares to minimize the integrated residuals over a quasi-flexible time mesh.}


%and the implementation of integrated residual methods for solving differential equations in the context of dynamic optimization will be described and analyzed. Additionally, a quasi-flexible time-meshing strategy will be proposed and we will show how can our method be used in optimization-based control applications.

%Using the integrated residuals method presents the opportunity to implement an advanced discretisation scheme capable of handling a finite number of discontinuities.

\begin{comment}
\hl{revisit this paragraph 
Choosing an appropriate mesh for the problem is a non-trivial task. Most of the results and studies present in the literature are focused towards the convergence behaviour of different mesh refinement schemes, or the consistency between the solution of the associated nonlinear programming problem (NLP) and continuous-time optimal control problem (OCP). In order to improve the accuracy of the approximation and converge to the exact analytical solution, one can either increase the degree of the approximating polynomial basis (p-methods) or increase the number of mesh intervals (h-methods). In regions where the solution is smooth, p-methods can achieve fast convergence with a relatively coarse mesh, while in regions with discontinuities or abrupt changes h-methods are very effective. To combine the best of both worlds, hp refinement has been proposed, but the convergence rate can be improved even further by adding mesh flexibility and introducing mesh nodes as decision variables in the NLP. However, to ensure the problem is well posed numerically, nodes are constrained to move only within a neighbourhood of the pre-defined equidistant mesh.    
%While these results are useful guidelines when selecting the locations of mesh nodes, fixed mesh have two fundamental disadvantages when dealing with discontinuities. Using the mesh points as decision variables in the optimization problem is a strategy insufficiently explored and yet with an enormous potential. 
} 
\end{comment}

% In contrast with off-the-shelf alternatives and traditional time-stepping methods for solving differential equations which can only be used inside a shooting method, the proposed solver tackles the OCPs with dynamics constraints as a single-step process and it includes all the decision variables in a single optimization problem. The main advantage of solving the OCPs in one go is the possibility to use previously computed information in order to improve the solution and the elegant and efficient manner of warm starting. 

%Evidence is provided to support our claims

%, one differential equation and one control problem regarded as an iterative sequence of feasibility problems.

%Methods used for ensuring constraint satisfaction n the works of [REF] and [REF] 


DE::

zagorowska.marta: Has this reformulation been used in the literature? It it has been used, we could just point to the reference. Otherwise, this bit raises some questions about how exactly the classic optimal control problem can be reformulated into our equations here.
Nov 8, 2021 3:40 PM
zagorowska.marta: One of Yuanbo's papers?

% In the particular case when initial and final time-points $t_0$ and $t_f$ are elements in $T$ (i.e.\ $\{t_0,t_f\} \in T$) the above functions become boundary constraints.

, but where $x$ includes the costate/adjoint variables and a multipoint BVP is solved to allow for discontinuous adjoints

%%%%%%%%%%%
\begin{comment}
\begin{equation}
    \dot{x}(t) = f(x(t), t), \quad \forall t \in \mathcal{T}
\label{eq:ode}
\end{equation}

and the dynamics function $f : \mathbb{R}^{N_x} \times \mathbb{R} \rightarrow \mathbb{R}^{N_x}$. In problems with algebraic equations, (\ref{eq:ode}) can be generalised as a system of

\begin{equation}
    0 = F(\dot{x}(t), x(t), u(t), t), \quad \forall t \in \mathcal{T}
\label{eq:dae}
\end{equation}
where and .

\begin{equation}
    \begin{aligned}
        \text{find} \quad & x(t), u(t)\\ %\min_{x,u} \quad & 0
        \textrm{s.t.} \quad & F(\dot{x}, x, u, t) = 0 \ \  \forall t\in[t_0,t_f]\\
                      & J(x,u,t)= J_i %\leq
    \end{aligned}
    \label{eq:feas_problem}
\end{equation}

where the cost bounds $J_i$ are selected according to bisection method or any other similar alternative. This can be interpreted as a construction of level curves and is useful in cases with a very complex function $F$. 

%\begin{subequations}
\begin{equation}
\begin{aligned}
        \min_{x(\cdot),u(\cdot)} \quad J(x,u)\\
\end{aligned}
\label{eq:cost}
\end{equation}
where $J$ is the cost functional, subject to the path constraints

 This formulation is common amongst optimal control, estimation and system identification problems.
 
 In optimal control, algebraic variables  are manipulated to control (\ref{eq:dae}) according to an optimality criterion, subject to constraints. This may be formulated as a Dynamic Optimisation Problem (DOP)
\end{comment}

NUMSOL::

%$\epsilon_R \in \mathbb{R}$,
%approximation error:
%\begin{equation}
%r_{\dot{x}}(t)=\norm{\tilde{\dot{x}}(t)-\dot{x}(t)}
%\end{equation}

% In order to \hl{perfectly} enforce the dynamics of the system in problem \hl{3} defined above, function $F$ has to be zero over the whole time interval $\mathcal{T}$ as stated in\hl{3b}. This leads to infinitely many constraints which cannot be handled in practice. To overcome this, 

%a set of equations:
%\begin{equation}
%    0=F(\tilde{x}(t), \dot{\tilde{x}}(t), \tilde{u}(t), t)
%    \label{eq:Residuals}
%\end{equation}

% The Euclidean  norm of $F$ 
% %\begin{equation}
% %    \epsilon_F (t)=\norm{F(\dot{\tilde{x}}(t), \tilde{x}(t), \tilde{u}(t), t)-F(\dot{x}(t), x(t), u(t), t)}_2^2,   \label{eq:Residuals}
% %\end{equation}
% %with $\epsilon_F : \mathcal{T} \to \mathbb{R}$ being 
% is the residual function used as integrand in \eqref{eq:approxErr} and can be interpreted as a measure of constraint violation for a particular time $t$ since the exact solution satisfies \eqref{eq:mainEq}. 

%Solving Eq. \eqref{eq:Residuals}
% In performing the transformation/transcription, one needs to select some approximation functions \hl{$\tilde{x} \in \mathbb{R}^{n}$, $\dot{\tilde{x}} \in \mathbb{R}^{m}$, $\tilde{u} \in \mathbb{R}^{p}$} for state, state derivative and control input respectively. These functions ($\tilde{x}$, $\dot{\tilde{x}}$ and $\tilde{u}$) are called basis functions and are parametrized by a finite number of decision variables \hl{$s^i_j$} and \hl{$c^i_j$}. %parameterized by 

% (otherwise we get asymptotic convergence of $\tilde{x}(\cdot)$ to $x(\cdot)$).

%and we perform a different approximation $\tilde{x}_i(t) \approx x(t) \quad \forall t \in \mathcal{T}_i$ on each mesh interval $i$. 

Really need sij eqn?

Convergence source?!



% \begin{figure}[h]%[!tbp]
% %%%%If you want to move this figure, move the whole figure environment
% \psfrag{x0}[][]{$x_0$}
% \psfrag{s1}[][]{$s^0_1$}
% \psfrag{s2}[][]{$s^0_2$}
% \psfrag{s3}[][]{$s^{0}_3$}
% \psfrag{xti}[][]{$\tilde{x}(t)$}
% \psfrag{t0}[][]{$t_0$}
% \psfrag{t10}[][]{$t^0_{1}$}
% \psfrag{t20}[][]{$t^0_{2}$}
% \psfrag{t30}[][]{$t^0_{3}$}
% \psfrag{t1}[][]{$t_1$}
% \psfrag{t11}[][]{}
% \psfrag{t21}[][]{}
% \psfrag{t31}[][]{}
% \psfrag{t2}[][]{$t_2$}
% \psfrag{tn}[][]{$t_{\tiny{N-1}}$}
% \psfrag{t1n}[][]{}
% \psfrag{t2n}[][]{}
% \psfrag{t3n}[][]{}
% \psfrag{tnn}[][]{$t_{\tiny{N}}$}
% \psfrag{t}[][]{$t$}
% \psfrag{xt0}[][]{$\tilde{x}_0$}
% \psfrag{xt1}[][]{$\tilde{x}_1$}
% \psfrag{xtn1}[][]{$\tilde{x}_{N-1}$}
% \psfrag{sp}[][]{$\shortparallel$}
% \psfrag{t40}[][]{$t^0_4$}
% \psfrag{t41}[][]{$t^1_4$}
% \psfrag{tnn1}[][]{$t^{N-1}_4$}
% \centering
% \includegraphics[width=0.48\textwidth]{Notationv2_arrows.pdf}
% \caption[Notation]{Notation version 2 \hl{superscript not appearing}}
%\label{fig:NotationArrows}
% \end{figure}


IRM :::
%The state continuity constraints and other fixed-point equality constraints in \eqref{eq:fixedplsq} can be included in the objective function as quadratic penalties in case one does not want to use the same decision variable for $\tilde{x}(t)$ at interval boundaries $t \in \{t_1,\dots,t_{N-1}\}$, as explained in the previous section. Since we are using $N$ intervals $[t_i, t_{i+1}]$ for defining basis functions, the integral in \eqref{eq:objlsq} can be split based on the locations of the nodes $t_i$. %Suppose we define a $N_F$-dimensional problem where the dynamics functional $F$ is defined as in \eqref{eq:dop}. We will denote by $F_k$ for $k \in \{1,\dots,N_F\}$ the $k\textsuperscript{th}$ component of $F$ ($F_k=F[k]$). This will enable us to expand the two-norm squared $\norm{F}^2_2$ as $\sum_{k=1}^{N_F}{F_k^2}$. 

%In collocation methods, error analysis can be a quite convoluted process, while in IRM we have a quantitative error measure already computed: the integrated residual
%\begin{equation}
%    \epsilon_R=\int_{t_0}^{t_{N}}{\sum_{d=1}^{D}{ F_d^2(\dot{x}_i(t),x_i(t),u_i(t),t)}}\diff t.
%    \label{eq:residerr}
%\end{equation} 

 %In plot \ref{fig:resid} \hl{showing the integrated residual for linear exponential $\dot{x}=-x$ example fixed vs flexible mesh} it can be observed that residuals are better spread over the whole time domain and the maximum residual value is lower in the case of quasi-flexible mesh. \hl{expand a bit more}
%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.85\columnwidth]{QuasiFlexibleMesh/residuals.pdf}
%    \caption{\hl{To edit. Residual distribution over the time domain: flexible in red, fixed in blue}}
%    \label{fig:resid}
%\end{figure}

% \begin{equation}
%     \epsilon_q=\Big|\epsilon_R-\sum_{i=0}^{N-1}{\sum_{k=1}^{Q}{w^i_k \cdot \norm{ F(\dot{\tilde{x}}(t^i_{Q,k}),\tilde{x}(t^i_{Q,k}),\tilde{u}(t^i_{Q,k}),t^i_{Q,k})}^2_2\Big|}}
% \end{equation} 


\begin{comment}
\begin{algorithm}
\SetAlgoLined
\KwResult{$x(t)$, $u(t)$}
 Set dynamics tolerance to $\epsilon_{F}$\;
 Set cost tolerance to $\epsilon_{J}$\;
 Initialize cost bound to $J_0$\;
 Set $J_{feasible}=\infty$\; 
 Set $J_{infeasible}=-\infty$\;
 
 \While{$J_{feasible}-J_{infeasible}\leq \epsilon_{J}$}{
  
  \begin{equation}
    \begin{aligned}
        R=\min_{x,u}  & \int_{t_0}^{t_f}{\norm{ F(\cdot,\cdot,t)}^2_2}\diff t + (J(\cdot,\cdot,t)-J_i)^2\\ %or I or IR
        %\textrm{s.t.} \quad & J(x,u,t)\leq J_i\\
        %& 0=F(\frac{\diff{x}}{\diff{t}},x,u,t)\\
        %& 0 \geq g(\frac{\diff{x}}{\diff{t}},x,u,t)
    \end{aligned}
    \label{eq:IRM}
  \end{equation}
  
  \eIf{$R\leq \epsilon_{F}$}{
    Update $J_{feasible}=J_i$\;
    Decrease $J_i$ (such that $J_{i+1} > J_{infeasible}$)\;
   }{
   Update $J_{infeasible}=J_i$\;
   Increase $J_i$ (such that $J_{i+1} < J_{feasible}$)\;
  }
 }
 \caption{Solving a sequence of problems using integrated residuals to enforce dynamics}
 \label{alg:seq_feas}
\end{algorithm}

problem \eqref{eq:qfexmesh} becomes  
\begin{equation}
    \begin{aligned}
    \min_{s,c,t_i} \quad & \sum_{i=0}^{N-1}{\sum_{l=1}^{q}{w_{l,i}\cdot\sum_{d=1}^{D}{ F_d^2(\dot{x}_i(t_{l,i}),x_i(t_{l,i}),u_i(t_{l,i}),t_{l,i})}}\diff t}\\
    \textrm{s.t.} \quad & J(x,u,t)\leq J_i\\
    \end{aligned}
    \label{eq:intro_dim}
\end{equation}

\end{comment}

p.falugi: you have a while loop and an index i that is never properly updated. Also the index i was used to split the time interval. Also check the optimization problem (14).   You should introduce the iterations there since you mention the you choose the cost iteratively


%If this is the case, we have just computed a valid suboptimal solution, otherwise we deal with an infeasible cost and we need to solve the problem again for a different, higher cost value.

perf:::
%But we degrade the computational time performance.%phi is like a tuning know trading off computational perf for accuracy

%in Figure \ref{fig:NotationFig3} can be seen the optimal

%%%%%%Fig31 is the initial one, slightly bigger
%%%%%%Fig32 is narrow to save space, from one of the comments
\begin{comment}
\begin{figure}[!tbp]
\centering
\psfragfig[width=0.48\textwidth]{Figures/Fig32}{
\psfrag{uti}[][]{$\tilde{u}(t)$}
\psfrag{uu}[][]{$u_U$}
\psfrag{ul}[][]{$u_L$}
\psfrag{t0}[][]{$t_{0}$}
\psfrag{t1}[][]{$t_1$}
\psfrag{t2}[][]{$t_2$}
\psfrag{t3}[][]{$t_3$}
\psfrag{t}[][]{$t$}
\psfrag{t1ms}[][]{\scriptsize{$t_0+\sigma_{-}$}}
\psfrag{t1ps}[][]{\scriptsize{$t_0+\sigma_{+}$}}
\psfrag{t2ms}[][]{\scriptsize{$t_1+\sigma_{-}$}}
\psfrag{t2ps}[][]{\scriptsize{$t_1+\sigma_{+}$}}
\psfrag{sp}[][]{$\shortparallel$}
\psfrag{t40}[][]{{$t_1^{*}$}}
\psfrag{t41}[][]{{$t_2^{*}$}}
\psfrag{tnn1}[][]{$t_{N}$}
}
\caption[Notation]{Solution for the control input $u$ to a double integrator problem \hl{ref} using fixed vs flexible mesh}
\label{fig:NotationFig3}
\end{figure}
\end{comment}


% \begin{figure}[!tbp]
% \psfrag{uti}[][]{$\tilde{u}(t)$}
% \psfrag{uu}[][]{$u_U$}
% \psfrag{ul}[][]{$u_L$}
% \psfrag{t0}[][]{$t_{0}$}
% \psfrag{t1}[][]{$t_1$}
% \psfrag{t2}[][]{$t_2$}
% \psfrag{t3}[][]{$t_3$}
% \psfrag{t}[][]{$t$}
% \psfrag{t1ms}[][]{{$t_1-\sigma$}}
% \psfrag{t1ps}[][]{{$t_1+\sigma$}}
% \psfrag{t2ms}[][]{{$t_2-\sigma$}}
% \psfrag{t2ps}[][]{{$t_2+\sigma$}}
% \psfrag{sp}[][]{$\shortparallel$}
% \psfrag{t40}[][]{{$t_1^{\#}$}}
% \psfrag{t41}[][]{{$t_2^{\#}$}}
% \psfrag{tnn1}[][]{$t_{N}$}
% \centering
% \includegraphics[width=0.48\textwidth]{Fig31.pdf}
% \caption[Notation]{Solid - flexible mesh, dashed - fixed mesh, dotted - analytic \hl{Can this figure be shrunk vetically to make space?}}
% \label{fig:NotationFig3}
% \end{figure}

%To gain a better understanding of the flexible mesh concept, we can consider the control input $\tilde{u}(\cdot)$ to a minimum-time repositioning example \cite[Section 4.14.3]{betts_practical_2010}. The exact analytical solution $u(\cdot)$ has a bang-bang structure, the numerical solution computed using pre-defined nodes $t_i$ and $N=3$ mesh intervals will be a while solid line depicts the numerical solution generated using flexible mesh approach and $N=3$ intervals.

%Optimal locations for nodes $t_1$ and $t_2$ as obtained from the solution of the optimization problem are denoted as $t_1^*$ and $t_2^*$.

perf::

% This allows us to state a general theorem emphasizing the strengths of our algorithm.
% \begin{observation}
% Let problem $\mathcal{P}$ be a generic dynamic optimization problem (DOP) of the form \eqref{eq:dop} with $F$ being a functional describing the dynamics constraints. Solving $\mathcal{P}$ using flexible mesh will give a solution with a residual error smaller or equal to the residual error obtained using a fixed mesh. 
%  \end{observation}

% \begin{proof}
% Consider the sample problems \eqref{eq:proof1} and \eqref{eq:proof2} below and observe that problem \eqref{eq:proof1} includes the original problem \eqref{eq:proof2} since the only difference stands in the variables that are optimized over. It is considered known that $f^\# \leq f^*$. 
% \begin{equation}
%     \begin{aligned}
%     f^\#=\min_{x,y} \quad & f(x,y)\\
%     \textrm{s.t.} \quad & g(x,y)\leq 0\\
%                         & h(x,y) = 0\\
%     \end{aligned}
%     \label{eq:proof1}
% \end{equation}
% \begin{equation}
%     \begin{aligned}
%     f^*=\min_{x} \quad & f(x,y)\\
%     \textrm{s.t.} \quad & g(x,y)\leq 0\\
%                         & h(x,y) = 0\\
%     \end{aligned}
%     \label{eq:proof2}
% \end{equation}

% It follows that the solution $\epsilon_R^\#$ to problem \eqref{eq:qfexmesh} is never higher than the solution $\epsilon_R^*$ to \eqref{eq:leastsq}. By looking at the objective function of both problems we can observe that it is exactly the same function as the residual error defined in \eqref{eq:approxErr}. Thus, the optimal point is $\epsilon_R^\#\leq\epsilon_R^*$. 
% \end{proof}

%\hl{talk about warm starting if time \& space}
\begin{comment}
To further improve the performance of our algorithm, when a new update for $J_{feasible}$ is found we will store the values for discrete decision variables $s$, $c$ and $t_i$ used to construct the continuous time solutions for $x(t)$ and $u(t)$ into variables called $s_{feasible}$, $c_{feasible}$ and $t_{i,feasible}$. When a new iteration of the algorithm \ref{alg:seq_feas} will run, these vectors will be used as initial guesses for the inner-loop as it is shown in algorithm \ref{alg:interes}. 
\begin{algorithm}
\SetAlgoLined
\KwResult{Integrated residual $\epsilon_R$}
 Initialize $s$, $c$ and $t_i$ with $s_{feasible}$ $c_{feasible}$ and $t_{i,feasible}$\;
 %\While{While condition}{
 % instructions\;
 % \eIf{condition}{
 %  instructions1\;
 %  instructions2\;
 %  }{
 %  instructions3\;
 % }
 %}
 \caption{Solving an integrated residual problem with warm-start}
 \label{alg:interes}
\end{algorithm}
\end{comment}

\end{comment}

\begin{comment}
abs::
\begin{comment}
\begin{abstract}
Handling dynamics constraints in optimization based control can be challenging due to nonlinearities and discontinuities that can appear in the differential equations modelling the system's behaviour as well as in the solution. Solving these problems using common time-marching schemes can lead to inefficiency and using typical mesh refinement procedures may even fail to reach the desired target accuracy in a reasonable amount of computational time. This paper introduces integrated residual method with quasi-flexible mesh as an alternative to existing non-adaptive mesh refinement schemes generally used in \hl{collocation} methods. Numerical examples show that our new method can give superlinear \hl{(cubic)} speed of convergence and the computational time can be up to five times lower when comparing an adaptive mesh approach to a fixed time-grid. The results show that even in complex real-life problems such as satellite reorientation, solutions of higher accuracy can be achieved.
\end{abstract}
\end{comment}




comm::
zagorowska.marta: A general structure of the abstract:
1. An introduction. Example: Solving optimal control problems is challenging because <nonlinearities, time, constraints, whatever>
2. What people do and why it doesn't work (aka problem statement). Example: Direct methods, such as collocation, are commonly used to solve optimal control problems. Collocation fails because <it is sensitive to discontinuities, something>
3. Contribution of the paper. Example: This paper <introduces> integrated residual method with quasi-flexible mesh as an alternative to collocation. It is shown that <something something>.
4. Actual outcomes. Example: Numerical examples show that the new method is XXX times better than collocation and gives JJJJJ time savings (I am absolutely creating random stuff here)
5. So what. Example: The results confirm that IRM is a good alternative to collocation.
Sep 10, 2021 6:36 PM
Hit Enter to reply
zagorowska.marta: In principle, the introduction should have the same structure as the abstract. 
1. Introduction as general as possible
2. What the paper is about (briefly, one sentence)
3. What people do and why it fails
4. Our contributions
5. A description of how the rest of the paper looks like "This paper is structured as follows..."
Sep 10, 2021 6:36 PM
zagorowska.marta: Maybe something like that would do: Dynamic optimisation problems are challenging to solve numerically because <of their complexity and implicit dependence on time>. In this paper, we propose a new numerical method to solve dynamic optimisation problems using integrated residuals methods with quasi-flexible time mesh.

Existing methods used in solving....<here goes the bit about collocation and why it fails, multiple shooting and why it fails, existing meshing and why it fails, time-marching bits as well>.

The main contribution of this paper is a new method based on integrated residuals that allows overcoming these drawbacks. Our approach relies on numerically integrating <here goes the bit why IRM is better than any other method>.

The paper is structures as follows <here goes a brief outline of what is in the paper>.

Yuanbo Nie: 1. I think collocation vs IRM is not really the key point of this paper. The flexible mesh should be the key selling point I think. 
2. It is not reallyh clear from the start what problems are we solving: differential equations? dynamic optimizations? I suggest to focus the main capability on solving differential inclusions and make the part on dynamic optimization an extension.
Oct 29, 2021 11:43 AM
Hit Enter to reply
Yuanbo Nie: This is too strong of an argument and generally I would say no method can really guarantee that.
Oct 29, 2021 11:45 AM
Hit Enter to reply
Yuanbo Nie: Are we demonstrating this in the paper? Otherwise may not be relevant. Abstract should quickly go to the key selling point of the paper
Oct 29, 2021 11:46 AM
Hit Enter to reply
Yuanbo Nie: We are not the first/only one to do this. The key point we have here is that we have combined flexible mesh with a method that takes good care of the error inbetween mesh intervals, i.e. the IRM.
Oct 29, 2021 11:51 AM
Yuanbo Nie: Only in this case flexible mesh makes sense
Oct 29, 2021 11:52 AM
Hit Enter to reply
Yuanbo Nie: This is more suitable for introduction. In abstract, we should say directly the results, e.g. from experiment experiements we obtain N time speedup for the same required accuracy.
Oct 29, 2021 11:55 AM
Hit Enter to reply
Yuanbo Nie: Make a clear distiction between differential equations and dynamic optimization problem. I would suggest to keep the main body of the text for the method developed in solving differential equations, and use extra paragraph and sections to extend its usage in solving dynamic optimization problems.
Oct 29, 2021 12:01 PM
Yuanbo Nie: The reason for this is because we are not really solving DOPs in our numerical examples, by assuming we know the  solution already

Ian McInerney: This seems very late in the abstract to actually introduce the paper contributions. You should generally try to do it in the first 3rd to make sure you capture the reader's attention.

Yuanbo Nie: Consider selling directly the benefits of the proposed method in abstract, instead of starting with the drawbacks of existing approach.

Yuanbo Nie: Make a clear distiction between differential equations and dynamic optimization problem. I would suggest to keep the main body of the text for the method developed in solving differential equations, and use extra paragraph and sections to extend its usage in solving dynamic optimization problems.
Oct 29, 2021 12:01 PM
Yuanbo Nie: The reason for this is because we are not really solving DOPs in our numerical examples, by assuming we know the  solution already

\begin{comment}
\begin{figure}[!tbp]
\centering
\psfragfig[width=0.48\textwidth]{Figures/Fig32}{
\psfrag{uti}[][]{$\tilde{u}(t)$}
\psfrag{uu}[][]{$u_U$}
\psfrag{ul}[][]{$u_L$}
\psfrag{t0}[][]{$t_{0}$}
\psfrag{t1}[][]{$t_1$}
\psfrag{t2}[][]{$t_2$}
\psfrag{t3}[][]{$t_3$}
\psfrag{t}[][]{$t$}
\psfrag{t1ms}[][]{\scriptsize{$t_0+\sigma_{-}$}}
\psfrag{t1ps}[][]{\scriptsize{$t_0+\sigma_{+}$}}
\psfrag{t2ms}[][]{\scriptsize{$t_1+\sigma_{-}$}}
\psfrag{t2ps}[][]{\scriptsize{$t_1+\sigma_{+}$}}
\psfrag{sp}[][]{$\shortparallel$}
\psfrag{t40}[][]{{$t_1^{*}$}}
\psfrag{t41}[][]{{$t_2^{*}$}}
\psfrag{tnn1}[][]{$t_{N}$}
}
\caption[Notation]{Solution for the control input $u$ to a double integrator problem \hl{ref} using fixed vs flexible mesh}
\label{fig:NotationFig3}
\end{figure}
\end{comment}

p.falugi: well if t_0 is fixed t_1 could be let to assume smaller values (the same applies for tf)


% Continuous-time dynamical systems can often be described by a system of ordinary differential equations (ODEs), differential-algebraic equations (DAEs) or the more general differential-algebraic inclusions (DAIs). 

\end{comment}
